The Highs and Lows of Simple Lexical Domain Adaptation Approaches for Neural Machine Translation

Machine translation systems are vulnerable to domain mismatch, especially in a low-resource scenario. Out-of-domain translations are often of poor quality and prone to hallucinations, due to exposure bias and the decoder acting as a language model. We adopt two approaches to alleviate this problem: lexical shortlisting restricted by IBM statistical alignments, and hypothesis re-ranking based on similarity. The methods are computationally cheap, widely known, but not extensively experimented on domain adaptation. We demonstrate success on low-resource out-of-domain test sets, however, the methods are ineffective when there is sufficient data or too great domain mismatch. This is due to both the IBM model losing its advantage over the implicitly learned neural alignment, and issues with subword segmentation of out-of-domain words.

==> latest_rerank_results.tex <==
BLEU, shortlist 10 10, rerank, law
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 20.8 53.1/27.6/16.7/10.7 (BP = 0.919 ratio = 0.922 hyp_len = 44409 ref_len = 48168)

BLEU, no shortlist, rerank, law
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 19.8 51.4/26.4/16.1/10.5 (BP = 0.906 ratio = 0.910 hyp_len = 43841 ref_len = 48168)

--------
BLEU, shortlist 10 10, rerank, it
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 17.8 38.0/20.1/13.6/9.7 (BP = 1.000 ratio = 1.048 hyp_len = 16951 ref_len = 16178)

BLEU, no shortlist, rerank, it
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 15.3 33.5/17.2/11.7/8.1 (BP = 1.000 ratio = 1.108 hyp_len = 17926 ref_len = 16178)
 
--------
BLEU, shortlist 10 10, rerank, all
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 18.8 43.4/22.2/15.1/11.4 (BP = 0.933 ratio = 0.936 hyp_len = 127430 ref_len = 136212)

BLEU, no shortlist, rerank, all
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 18.4 40.2/20.7/14.4/11.0 (BP = 0.966 ratio = 0.967 hyp_len = 131684 ref_len = 136212)
 
--------
BLEU, shortlist 10 10, rerank, medical
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 57.6 77.3/62.6/53.7/47.6 (BP = 0.971 ratio = 0.971 hyp_len = 17506 ref_len = 18026)

BLEU, no shortlist, rerank, medical
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 60.4 78.7/65.1/56.7/51.2 (BP = 0.972 ratio = 0.973 hyp_len = 17536 ref_len = 18026)
 
--------
BLEU, shortlist 10 10, rerank, koran
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 1.0 22.9/2.8/0.4/0.1 (BP = 0.862 ratio = 0.871 hyp_len = 31870 ref_len = 36605)

BLEU, no shortlist, rerank, koran
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 0.9 20.2/2.2/0.3/0.1 (BP = 0.907 ratio = 0.911 hyp_len = 33355 ref_len = 36605)
 
--------
BLEU, shortlist 10 10, rerank, subtitles
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 2.8 26.0/5.0/1.4/0.4 (BP = 0.956 ratio = 0.957 hyp_len = 16487 ref_len = 17235)
 
BLEU, no shortlist, rerank, subtitles
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.10 = 2.4 21.4/3.7/1.1/0.4 (BP = 1.000 ratio = 1.100 hyp_len = 18953 ref_len = 17235)


--------
--------
BLEU, no shortlist law
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 17.8 53.0/27.5/16.9/11.0 (BP = 0.778 ratio = 0.799 hyp_len = 38490 ref_len = 48168)
BLEU, shortlist law
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 19.3 56.1/29.4/17.9/11.4 (BP = 0.804 ratio = 0.821 hyp_len = 39544 ref_len = 48168)
BLEU, no shortlist it
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 15.7 34.6/18.8/13.1/9.5 (BP = 0.930 ratio = 0.932 hyp_len = 15083 ref_len = 16178)
BLEU, shortlist it
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 18.0 43.9/24.7/17.1/12.1 (BP = 0.828 ratio = 0.841 hyp_len = 13606 ref_len = 16178)
BLEU, no shortlist all
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 17.5 43.7/23.7/17.0/13.3 (BP = 0.797 ratio = 0.815 hyp_len = 111036 ref_len = 136212)
BLEU, shortlist all
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 18.1 48.1/25.7/18.0/13.7 (BP = 0.771 ratio = 0.793 hyp_len = 108062 ref_len = 136212)
BLEU, no shortlist medical
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 61.4 82.3/68.8/60.2/54.2 (BP = 0.936 ratio = 0.938 hyp_len = 16916 ref_len = 18026)
BLEU, shortlist medical
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 58.2 80.0/65.4/56.3/49.7 (BP = 0.940 ratio = 0.942 hyp_len = 16977 ref_len = 18026)
BLEU, no shortlist koran
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 0.8 21.5/2.4/0.4/0.1 (BP = 0.636 ratio = 0.689 hyp_len = 25212 ref_len = 36605)
BLEU, shortlist koran
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 0.9 25.3/3.1/0.4/0.1 (BP = 0.615 ratio = 0.673 hyp_len = 24628 ref_len = 36605)
BLEU, no shortlist subtitles
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 2.6 24.6/4.6/1.4/0.4 (BP = 0.898 ratio = 0.902 hyp_len = 15554 ref_len = 17235)
BLEU, shortlist subtitles
BLEU+case.mixed+numrefs.1+smooth.exp+tok.13a+version.1.4.14 = 2.8 29.8/5.8/1.8/0.6 (BP = 0.767 ratio = 0.791 hyp_len = 13626 ref_len = 17235)

